lpNTK: Better Generalisation with Less Data via Sample Interaction During Learning

Although much research has been done on proposing new models or loss functions to improve the generalisation of artificial neural networks (ANNs), less attention has been directed to the impact of the training data on generalisation. In this work, we start from approximating the interaction between samples, i.e. how learning one sample would modify the model's prediction on other samples. Through analysing the terms involved in weight updates in supervised learning, we find that labels influence the interaction between samples. Therefore, we propose the labelled pseudo Neural Tangent Kernel (lpNTK) which takes label information into consideration when measuring the interactions between samples. We first prove that lpNTK asymptotically converges to the empirical neural tangent kernel in terms of the Frobenius norm under certain assumptions. Secondly, we illustrate how lpNTK helps to understand learning phenomena identified in previous work, specifically the learning difficulty of samples and forgetting events during learning. Moreover, we also show that using lpNTK to identify and remove poisoning training samples does not hurt the generalisation performance of ANNs.

==> authorship.tex <==
\makeatletter
\newcommand{\myfnsymbol}[1]{%
  \expandafter\@myfnsymbol\csname c@#1\endcsname
}
% Mapping of how the \thanks symbols will be interpreted sequentially
\newcommand{\@myfnsymbol}[1]{%
  \ifcase #1
    % 0
  \or 1% 1
  \or 2% 2
  \or 3
  \or 4
  \or 5
  \or \TextOrMath{\textdagger}{\dagger}% 7
  \or \TextOrMath{\textdaggerdbl}{\ddagger}%8
  \fi
}
% Just to make things explicit in the code what it means
\newcommand{\sg}{\@myfnsymbol{1}}
\newcommand{\yr}{\@myfnsymbol{2}}
\newcommand{\sa}{\@myfnsymbol{3}}
\newcommand{\ks}{\@myfnsymbol{4}}
\newcommand{\uoe}{\@myfnsymbol{6}}
\newcommand{\ubc}{\@myfnsymbol{7}}
\newcommand{\intern}{\@myfnsymbol{8}}
\def\thanks#1{\protected@xdef\@thanks{\@thanks
    \protect\footnotetext{#1}}
}

\makeatother


==> sections/active_learning.tex <==
\section{(?) Use Case 3: Active Learning}
\label{sec:active}

==> sections/exploration_drl.tex <==
\section{Use Case 2: Exploration in Deep Reinforcement Learning}
\label{sec:drl}

Beyond the supervised learning discussed in Section~\ref{sec:image}, we also explore the effectiveness of our method on reinforcement learning where no immediate supervision signal is available for the learning of the models (a.k.a. agents).

\subsection{Derivation on Deep Q-Network}
\label{ssec:drl:drivation}

Following \cite{mnih2015dqn}, we use DQN as the agent to learn the optimal policy in the Atari environments modelled as finite Markov decision processes, of which each is constituted by the following terms:
1) a set of states $\sS$;
2) a set of actions $\sA$;
3) a reward function $r:\sS\times\sA\rightarrow\sR$;
4) a transmission probability $p(\vs', r|\vs, a)$.
Our agent is a Q-function parameterised by an ANN, i.e. $Q(\vs, a; \vw):\sS\times\sA\rightarrow\sR$, and the objective of learning is to maximise the expected discounted return $G=\sum_{t=1}^{T} r(\vs_t, a_t)$.
To achieve the learning objective, our agent would first interact with the environments and store the collected transitions $\left\{ \vs, a, \vs', r\right\}$ into the replay buffer.
We then sample a batch of transitions $\sB=\left\{\vs, a, \vs', r\right\}$, and update the parameters through minimising a mean squared error function defined as $\gL = \frac{1}{|B|}\sum_{(\vs,a,\vs',r)\in B} \frac{1}{2}\delta^2$ where $\delta\triangleq Q(\vs,a) - \left(r + \gamma\max_{a'}Q(\vs',a')\right)$ is known as the temporal difference (TD) error.

Suppose we roll out a transition $(\su, \au, r, \vs')$ at time-step $t$, and we can approximate the change of Q-estimation on another state-action pair, i.e. $\Delta Q^t(\so, \ao)$, by first-order Taylor approximation shown below:
\begin{equation}
    \begin{aligned}
        \Delta_{(\su, \au)}Q(\so, \ao) 
        & \triangleq  Q^{t+1}(\so, \ao) - Q^{t}(\so, \ao) \\
        & \approx \eta \cdot \mK^t_{\ao,\au}(\so, \su) 
        \cdot \underbrace{\left( r + \gamma\max_{a'} Q^t(\vs', a') - Q^t(\su, \au) \right)}_{\text{TD error}}
    \end{aligned}
    \label{eq:drl:drivation}
\end{equation}
where $\eta$ and $\mK$ are defined in the same way as in Equation~\ref{eq:lpntk:approx}, and $\mK^t_{\ao,\au}$ refers to the element in the row $\ao$ and column $\au$ of $\mK^t$.

More details about the above derivation are provided in Appendix~\ref{appsec:drl}.

\subsection{Exploration Strategy following lpNTK}
\label{ssec:drl:exploration}

Following the above derivation, it is straightforward to see that the three types of relationships illustrated in Section~\ref{sec:rethinking} also hold for state-action pairs in DRL.
However, in this case, the role of label is replaced with the actions chose by the agent as shown by the subscripts of $\mK$, and the feature representation is not a sum but rather arow of $\nabla_\vw Q(\vs)$.
Formally, the lpNTK for DQN can be defined as:
\begin{equation}
    \begin{aligned}
        \text{lpNTK}((\so, \ao), (\su, \ao))
        & \triangleq \sum \left[ \vs(\au) \cdot \vs(\ao)\tp \right] \odot \mK(\so,\su) \\
        & = \underbrace{\left[ \vs(\ao)\tp \nabla_{\vw}Q(\so) \right]}_{1 \times d}
        \cdot
        \underbrace{\left[\nabla_{\vw}Q(\su)\tp \vs(\au)\right]}_{d\times 1}
    \end{aligned}
    \label{eq:drl:exploration:lpntk_definition}
\end{equation}
where $\vs(a)$ is a one-hot vector of which only the $a$-th element is $1$.

Inspired by the results on debasing supervised learning datasets in Section~\ref{ssec:image:poisoning_exp}, we argue that using lpNTK as an exploration strategy for DRL agents could also help to improve the expected return of the learnt policy.
Similar to the supervised learning case where interchangeable samples are more important when there are just a few data and unrelated/contradictory samples are more important are there are enough data, we propose that the DQN agents should explore state-action pairs that are more interchangeable with the replay buffer at the beginning of learning.
Following this heuristic, we propose the following exploration strategy which we refer to as ``lpNTK-max'':
\begin{proposition}
Suppose the parameters of Q-network will be updated with a batch of state-action pairs $\{(\vs_1, a_1), (\vs_2, a_2), \dots, (\vs_n, a_n)\}$ at time-step $t+1$, and the current state is $\vs$, the action $a$ to choose should be the one that is \textbf{the most interchangeable} to the batch of state-action pairs, i.e., maximizes the average similarity between $(\vs, a)$ and $\{(\vs_i, a_i)$ for $i\in\{1, \dots, n\}$, as follows:
\begin{equation}
    a = \arg\max_a \frac{1}{n}\sum_{i=1}^{n} \gK^{t} \left((\vs, a), (\vs_i, a_i)\right).
    \label{eq:drl:explroation:ntk_max}
\end{equation}
\label{strategy:drl:exploration}
\end{proposition}

During the learning, we would use the following behaviour policy:
\begin{equation}
    a =
    \begin{cases}
      \arg\max_a Q(\vs, a), & \text{with probability}\ 1-\epsilon \\
      \text{Strategy 1},   & \text{with probability}\ \epsilon 
    \end{cases}
    \label{eq:ntk_greedy_policy}
\end{equation}

\subsection{Experiment Results}
\label{ssec:drl:exp}

To verify the effectiveness of the above \textbf{Strategy 1}, we compare the above strategy with the $\epsilon$-greedy strategy in Atari games including Enduro, SpaceInvaders, and Freeway, and the validation returns of policies obtained via these two strategies are shown in the Table~\ref{tab:drl:exp:return_mean_std} below.

\begin{table}[!h]
\centering
\begin{tabular}{c|ccc}
\hline
Games     & Enduro              & SpaceInvaders      & Freeway         \\ \hline
e-greedy  & $1199.11\pm227.37$  & $302.87\pm 143.60$ & $27.55\pm 1.34$ \\ \hline
lpNTK-max & $1674.55\pm 421.02$ & $316.8\pm 153.41$  & $28.68\pm 1.43$ \\ \hline
\end{tabular}
\caption{
Validation return of different exploration strategies on the selected Atari environments.
We run the experiment with $3$ different random seeds, and the averaged return as well as the corresponding standard deviation are both given in the table above.
}
\label{tab:drl:exp:return_mean_std}
\end{table}

As show above, the validation return of lpNTK-max on all of the three environments are higher than the $\epsilon$-greedy strategy. 
Note that the only difference between our exploration strategy given in Equation~\ref{eq:drl:explroation:ntk_max} and the $\epsilon$-greedy is that we replace the random selection with our lpNTK method illustrated in Strategy~\ref{strategy:drl:exploration}.
However, one problem we found during this experiment is that our method cannot help across all environments, i.e. $\epsilon$-greedy can obtain similar performance to our lpNTK-max.
We argue that this also relates to the difficulty of the environments, and a full understanding of this problem may require more study in the future and is out of the scope of this work.

Overall, through Section~\ref{sec:image} and~\ref{sec:drl}, we show that our lpNTK can help to improve the generalisation performance which is measured by:
1) test accuracy in classification;
2) validation return in DRL.

